Large Language Models for Anomaly and Out-of-Distribution Detection: A Survey

Detecting anomalies or out-of-distribution (OOD) samples is critical for maintaining the reliability and trustworthiness of machine learning systems. Recently, Large Language Models (LLMs) have demonstrated their effectiveness not only in natural language processing but also in broader applications due to their advanced comprehension and generative capabilities. The integration of LLMs into anomaly and OOD detection marks a significant shift from the traditional paradigm in the field. This survey focuses on the problem of anomaly and OOD detection under the context of LLMs. We propose a new taxonomy to categorize existing approaches into two classes based on the role played by LLMs. Following our proposed taxonomy, we further discuss the related work under each of the categories and finally discuss potential challenges and directions for future research in this field. We also provide an up-to-date reading list of relevant papers.

==> explanation.tex <==
\section{LLMs for Explanation}
\label{sec:explanation}
Due to their remarkable capabilities in understanding and generating human-like text, LLMs have been explored for providing insightful explanations and analyses for anomaly and OOD detection results, thereby aiding in further planning, problem-solving and decision-making.

For applications in safety-critical domains, such as autonomous driving, providing explanations to stakeholders of AI systems has become an ethical and regulatory requirement \cite{li2023survey}. Consequently, there is a growing interest in developing explainable video anomaly detection frameworks. Holmes-VAD \cite{zhang2024holmes}, for instance, trains a lightweight temporal sampler to select frames with high anomaly scores and then employs an LLM to generate detailed explanatory analyses, offering clear insights into the detected anomalies. VAD-LLaMA \cite{lv2024video} generates instruction-tuning data to train only the projection layer of Video-LLaMA, enabling more comprehensive explanations of anomalies. AnomalyRuler \cite{yang2024follow} emphasizes a rule-based reasoning strategy with efficient few-normal-shot prompting, allowing for rapid adaptation to different VAD scenarios while providing interpretable, rule-driven explanations.  

Moreover, with the powerful capabilities of LLMs in understanding instructions and self-planning to solve tasks, an emerging research direction is to build autonomous agents based on LLMs to guide decision-making after anomalies or OOD are detected. For instance, AESOP \cite{sinha2024real} employs the autoregressive generation of an LLM to provide a zero-shot assessment of whether interventions are needed for the robotic system after an anomaly is detected.
